Retrieval-Based Transformer for Table Augmentation

Data preparation, also called data wrangling, is considered one of the most expensive and time-consuming steps when performing analytics or building machine learning models. Preparing data typically involves collecting and merging data from complex heterogeneous, and often large-scale data sources, such as data lakes. In this paper, we introduce a novel approach toward automatic data wrangling in an attempt to alleviate the effort of end-users, e.g. data analysts, in structuring dynamic views from data lakes in the form of tabular data. We aim to address table augmentation tasks, including row/column population and data imputation. Given a corpus of tables, we propose a retrieval augmented self-trained transformer model. Our self-learning strategy consists in randomly ablating tables from the corpus and training the retrieval-based model to reconstruct the original values or headers given the partial tables as input. We adopt this strategy to first train the dense neural retrieval model encoding table-parts to vectors, and then the end-to-end model trained to perform table augmentation tasks. We test on EntiTables, the standard benchmark for table augmentation, as well as introduce a new benchmark to advance further research: WebTables. Our model consistently and substantially outperforms both supervised statistical methods and the current state-of-the-art transformer-based models.

==> alt_tables.tex <==
\iffalse
\begin{table}[!htb]
\centering
\begin{tabular}{l|rr}
%\hline
 \multicolumn{3}{c}{\textbf{Row Population}} \\
& EntiTables & WebTables \\
\hline
BM25 & 54.44 & 41.16{\small $\pm$1.06} \\
DTR (initial) & 74.34 & 47.88{\small $\pm$1.10} \\
DTR (with RATA) & \textbf{80.26} & \textbf{49.62}{\small $\pm$1.11} \\
\hline
\multicolumn{3}{c}{\textbf{Column Population}} \\
& EntiTables & WebTables \\
\hline
BM25 & 62.93 & 84.17 \\
DTR after initial training & \textbf{90.07} & \textbf{94.91} \\
DTR after RATA training & \textbf{90.97} & \textbf{94.94} \\
% TODO: test significance (probably not)
\hline
\multicolumn{3}{c}{\textbf{Cell Filling}} \\
& EntiTables & WebTables \\
\hline
BM25 & 28.98 & 38.78 \\
DTR after initial training & 34.78 & \textbf{40.80} \\
DTR after RATA training & \textbf{37.48} & 40.26 \\
\hline
\end{tabular}
\caption{Retrieval answer-bearing MRR (\%)}
\label{tab:all_tasks_retrieval}
\end{table}
\fi

\iffalse
\begin{table}[!htb]
\centering
\begin{tabular}{l|rr}
\hline
& EntiTables & WebTables \\
\hline
BM25 & 54.44{\small $\pm$2.72} & 41.16{\small $\pm$1.06} \\
DTR after initial training & 74.34{\small $\pm$2.39} & 47.88{\small $\pm$1.10} \\
DTR after RATA training & \textbf{80.98}{\small $\pm$2.17} & \textbf{49.62}{\small $\pm$1.11} \\
\hline
\end{tabular}
\caption{Retrieval answer-bearing MRR (\%) for row population}
\label{tab:row_pop_retrieval}
\end{table}

\begin{table}[!htb]
\centering
\begin{tabular}{l|rr}
\hline
& EntiTables & WebTables \\
\hline
BM25 & 62.93{\small $\pm$2.73} & 84.17 {\small $\pm$0.65} \\
DTR after initial training & \textbf{90.07}{\small $\pm$1.79} & \textbf{94.91}{\small $\pm$0.41} \\
DTR after RATA training & \textbf{90.97}{\small $\pm$1.72} & \textbf{94.94}{\small $\pm$0.41} \\
% TODO: test significance (probably not)
\hline
\end{tabular}
\caption{Retrieval answer-bearing MRR (\%) for column population}
\label{tab:col_pop_retrieval}
\end{table}

\begin{table}[!htb]
\centering
\begin{tabular}{l|rr}
\hline
& EntiTables & WebTables \\
\hline
BM25 & 28.98 & 38.78 \\
DTR after initial training & 34.78 & \textbf{40.80} \\
DTR after RATA training & \textbf{37.48} & 40.26 \\
\hline
\end{tabular}
\caption{Retrieval answer-bearing MRR (\%) for cell filling.}
\label{tab:cell_filling_retrieval}
\end{table}
\fi
